AutoAlignV2: Deformable Feature Aggregation for Dynamic Multi-Modal 3D Object Detection

Point clouds and RGB images are two general perceptional sources in autonomous driving. The former can provide accurate localization of objects, and the latter is denser and richer in semantic information. Recently, AutoAlign presents a learnable paradigm in combining these two modalities for 3D object detection. However, it suffers from high computational cost introduced by the global-wise attention. To solve the problem, we propose Cross-Domain DeformCAFA module in this work. It attends to sparse learnable sampling points for cross-modal relational modeling, which enhances the tolerance to calibration error and greatly speeds up the feature aggregation across different modalities. To overcome the complex GT-AUG under multi-modal settings, we design a simple yet effective cross-modal augmentation strategy on convex combination of image patches given their depth information. Moreover, by carrying out a novel image-level dropout training scheme, our model is able to infer in a dynamic manner. To this end, we propose AutoAlignV2, a faster and stronger multi-modal 3D detection framework, built on top of AutoAlign. Extensive experiments on nuScenes benchmark demonstrate the effectiveness and efficiency of AutoAlignV2. Notably, our best model reaches 72.4 NDS on nuScenes test leaderboard, achieving new state-of-the-art results among all published multi-modal 3D object detectors. Code will be available at https://github.com/zehuichen123/AutoAlignV2.

==> tables/waymo_val.tex <==
\begin{table*}[hbpt]
    \centering
    \label{tab::waymores}
    \setlength{\tabcolsep}{1.6mm}
    \begin{tabular}{c | c|cc|cc|cc|cc}
    \toprule
    \multirow{2}{*}{Method} &
    \multirow{2}{*}{AutoAlignV2} &
    \multicolumn{2}{c|}{Vehicle L1/L2} &
    \multicolumn{2}{c|}{Pedestrian L1/L2} &
    \multicolumn{2}{c|}{Cyclist L1/L2} &
    \multicolumn{2}{c}{Overall L1/L2} \\
       &  & AP & APH & AP & APH & AP & APH & AP & APH\\     
	\midrule
	\midrule
    \multirow{2}*{SECOND} &  & 69.3/60.6 & 68.7/60.2 & 70.3/61.8 & 62.0/54.3 & 64.0/61.5 & 62.8/60.4 & 67.9/64.5 & 61.3/58.3\\
      & \checkmark & \textbf{70.1/61.3} & \textbf{69.5/60.9} & \textbf{72.1/63.5} & \textbf{63.8/56.0} & \textbf{67.0/64.3} & \textbf{65.8/63.1} & \textbf{69.6/66.3} & \textbf{63.0/60.0}\\
    \midrule
	\multirow{2}*{CenterPoint} &  & 69.3/60.6 & 68.7/60.2 & 70.3/61.8 & 62.0/54.3 & 64.0/61.5 & 62.8/60.4 & 67.9/64.5 & 61.3/58.3\\
      & \checkmark & \textbf{70.1/61.3} & \textbf{69.5/60.9} & \textbf{72.1/63.5} & \textbf{63.8/56.0} & \textbf{67.0/64.3} & \textbf{65.8/63.1} & \textbf{69.6/66.3} & \textbf{63.0/60.0}\\
    \bottomrule
    \end{tabular}
    \vskip 0.5em
    \caption{AP performance on different 3D object detectors w/o and w/ AutoAlignV2 on WOD validation set.}
    \label{tab:waymo_val}
\end{table*}
